AS2T: Arbitrary Source-To-Target Adversarial Attack on Speaker Recognition Systems

Recent work has illuminated the vulnerability of speaker recognition systems (SRSs) against adversarial attacks, raising significant security concerns in deploying SRSs. However, they considered only a few settings (e.g., some combinations of source and target speakers), leaving many interesting and important settings in real-world attack scenarios alone. In this work, we present AS2T, the first attack in this domain which covers all the settings, thus allows the adversary to craft adversarial voices using arbitrary source and target speakers for any of three main recognition tasks. Since none of the existing loss functions can be applied to all the settings, we explore many candidate loss functions for each setting including the existing and newly designed ones. We thoroughly evaluate their efficacy and find that some existing loss functions are suboptimal. Then, to improve the robustness of AS2T towards practical over-the-air attack, we study the possible distortions occurred in over-the-air transmission, utilize different transformation functions with different parameters to model those distortions, and incorporate them into the generation of adversarial voices. Our simulated over-the-air evaluation validates the effectiveness of our solution in producing robust adversarial voices which remain effective under various hardware devices and various acoustic environments with different reverberation, ambient noises, and noise levels. Finally, we leverage AS2T to perform thus far the largest-scale evaluation to understand transferability among 14 diverse SRSs. The transferability analysis provides many interesting and useful insights which challenge several findings and conclusion drawn in previous works in the image domain. Our study also sheds light on future directions of adversarial attacks in the speaker recognition domain.

==> attack.tex <==

\section{Adversarial Attack}\label{sec:attack}
In this section, we summarize several representative attacks from two dimension: 
the level of knowledge attacks rely on (white-box and black-box attacks) 
% and attack medium (digital and over-the-air attacks).
and attack medium (API and over-the-air attacks).

Note that although a plethora of adversarial attacks have been proposed, 
most of them are primarily studied in computer vision~\cite{akhtar2018threat},
and it is largely unknown if they can successfully be ported to all the recognition tasks due to the unique property of SR~\cite{chen2019real}.
Hence, in this work, we present three representative white-box attacks
% and two black-box attacks 
and two query-based attacks 
which have been demonstrated to be effective on at least one recognition task.

\subsection{White-box Attacks}
Most white-box attacks craft adversarial examples by gradient descent/ascent 
in which the gradient is obtained by backpropagation.

% \subsubsection{White-box Attacks}

\noindent {\bf Fast Gradient Sign Method (FGSM)}~\cite{goodfellow2014explaining}. 
FGSM perturbs an input $x$ by performing one-step gradient ascent to maximize a loss
function. Formally, a potential adversarial example is:
% \begin{align*}
%     \hat{x} = x + \varepsilon \times \emph{sign}(\nabla_x J(x,y))
% \end{align*}
\begin{center}
$\hat{x} = x + \varepsilon \times \emph{sign}(\nabla_x f(x,y))$
\end{center}
% \begin{center}
%     $\hat{x} = x + \varepsilon \times \emph{sign}(\nabla_x L(f(x),y))$
% \end{center}
where $\varepsilon$ is the step size of gradient ascent and
$f(x,y)$ is the loss function describing the cost of classifying $x$ as label $y$.
% $L(f(x),y)$ is the loss function describing the cost of classifying $x$ as label $y$.
% $L(f(x),y)$ is the loss function describing the cost of model $f(\cdot)$ to classify $x$ as label $y$.
% $J(x,y)$ is the loss function describing the cost of classifying $x$ as label $y$.

\smallskip
\noindent {\bf Projected Gradient Descent (PGD)}~\cite{madry2017towards}. PGD is an iterative version of FGSM. In each iteration, PGD applies FGSM with a small step size $\alpha$ and clips the result to ensure that it stays within an $\varepsilon$-neighborhood of the original input $x$. The intermediate example after the $i$-th iteration is:
% \begin{align*}
% x^i = \emph{clip}_{x,\varepsilon}(x^{i-1} + \alpha \times \emph{sign}(\nabla_x J(x^{i-1},y)))
% \end{align*}
\begin{center}
$x^i = \emph{clip}_{x,\varepsilon}(x^{i-1} + \alpha \times \emph{sign}(\nabla_x f(x^{i-1},y)))$
\end{center}
% \begin{center}
%     $x^i = \emph{clip}_{x,\varepsilon}(x^{i-1} + \alpha \times \emph{sign}(\nabla_x L(f(x^{i-1}),y)))$
% \end{center}
Note that PGD attack starts from a randomly perturbed example rather than the original example, which helps the attack find a better local minimum.
We denote by PGD-$x$ the PGD attack with $x$ steps for iteration,
the larger $x$, the stronger the adversarial examples.

\smallskip
\noindent {\bf CW}~\cite{carlini2017towards}. 
CW is introduced to search for adversarial examples with small magnitude of perturbations.
It formulates finding adversarial examples as an optimization problem 
whose objective function is the trade-off (controlled by a factor $c$) 
between the effectiveness and imperceptibility of adversarial examples. 
The effectiveness is measured by a loss function $f(x,y)$ such that $f(x,y)\leq 0$ if and only if the attack succeeds. 
% The effectiveness is measured by a loss function $L(f(x),y)$ such that $L(f(x),y)\leq 0$ if and only if the attack succeeds. 
The imperceptibility can be instantiated by $L_0$, $L_2$, and $L_\infty$ distance between adversarial and original examples, 
leading to three versions of CW attack, denoted by CW$_0$, CW$_2$, and CW$_{{\infty}}$, respectively. 
CW attack is equipped with a parameter $\kappa$, and 
the larger $\kappa$ is, the stronger the adversarial examples are.
We denote by CW$_p$-$x$ the CW$_p$ attack with $\kappa=x$.

\subsection{Black-box Attacks}
% Black-box attack can be divided into query-based and transfer-based attacks 
% based on whether the adversary can make adaptive queries to models.
According to whether an adversary can issue adaptive oracle queries to models, 
black-box attack can be broadly grouped into query-based and transfer-based attacks.

\subsubsection{Query-based}
% Indeed, query-based attack can be further divided into score-based and decision-based attacks based on the outputs returned by models in response to the queries.
% Although decision-based attack is obviously more challenging than score-based one, we are not aware of any decision-based attack shown effective on SRSs,
% thus we only focus on score-based attack in this work.
Depending on what type of outputs is provided by the model to an adversary in response to his probed inputs, 
query-based attack can be further divided into score-based and decision-based attacks.
While score-based attack can observe continous confidence scores, 
decision-based attack is restricted to discrete hard-label decisions, a stricter and more challenging case. 
Since we are not aware of any decision-based attack demonstrated effective on SRSs, in this work, 
we only focus on score-based attack.

Under black-box constraint, 
% Under black-box restriction, 
% although the gradient computation through backpropagation is prohibited, 
although an adversary is not permitted to compute the actual gradient via backpropagation, 
% the adversary can either estimate the gradient through queries or exploit gradient-free optimization approaches 
% the adversary can exploit either the gradient estimation techniques, e.g., Natural Evolution Strategy (NES) in FAKEBOB 
% or gradient-free optimization approaches, e.g., Particle Swarm Optimization (PSO) in SirenAttack. 
he can utilize either gradient estimation techniques, e.g., Natural Evolution Strategy (NES) in FAKEBOB, 
or gradient-free optimization approaches, e.g., Particle Swarm Optimization (PSO) in SirenAttack. 

\noindent {\bf FAKEBOB}~\cite{chen2019real}. 
FAKEBOB is similar to PGD except that it estimates gradients via NES  
and the attack starts from the original input voice instead of a randomly perturbed one.
Specifically, NES first creates $m$ noisy examples by adding Gaussian noises onto an example.
Then, the values of the loss function of $m$ examples are obtained by querying the model, which are finally exploited to approximate the gradient. 
FAKEBOB adopts an early-stop strategy to reduce the number of queries, i.e., stop searching once an adversarial example is found.
Similar to the CW attack, FAKEBOB also provides an option to control the confidence of adversarial examples via
a parameter $\kappa$. Furthermore, FAKEBOB proposed the first algorithm to estimate the threshold for SV and OSI tasks.


% Although particle swarm optimization has been adopted to conduct black-box attacks on speaker recognition~\cite{du2020sirenattack},
% it is significantly less effective than FAKEBOB~\cite{chen2019real}. Thus, we do not consider in this work.
% \noindent {\bf Particle Swarm Optimization (PSO).} TO DO.
\smallskip\noindent {\bf SirenAttack}~\cite{du2020sirenattack}.
SirenAttack searches for adversarial examples by leveraging PSO~\cite{PSO}, a gradient-free optimization method.
PSO imitates the behaviour of a swarm of birds. 
Each particle is a candidate solution,
and is iteratively updated via the weighted linear combination of three parts, i.e., inertia, local best solution and global best solution.
When the algorithm terminates, global best solution is the adversarial example we find.

\subsubsection{Transfer-based}
% Transfer-based attack generate adversarial examples on a local source model by white-box attack strategies mentioned above 
% % and transfer them to the remote target model which is probably also deceived by these adversarial examples.
% and present them to the remote target model which probably misbehaves on these malicious inputs. 
% The attack success rate of transfer-based attack largely depends on the similarity between the source and target models.
% When the gap between them is larger, the transferability rate is limited~\cite{chen2019real}.
Transfer-based attack generate adversarial examples on a local source model 
and present them to the remote target model which will probably misbehave on these malicious inputs. 
Since the local source model is totally transparent to the adversary, 
he can leverage any aforementioned white-box attack strategies. 
However, the attack success rate of transfer-based attack largely depends on the similarity between the source and target models.
When the gap between them is large, the transferability rate is limited~\cite{chen2019real}.


% \subsection{Physical Attacks}
\subsection{Over-the-air Attack}
% The adversarial voices can be passed to SR models over different mediums, 
% including over-the-line, over-the-air, over-the-radio, over-telephony-network and so on.
% Over-the-line attack feeds crafted adversarial voices in the form of audio file to the SR models directly via exposed API, 
% thus it will not introduce any disruption to adversarial voices.
% Over-the-air, over-the-radio and over-telephony-network are more practical attack scenarios 
% where adversarial voices are played by loudspeakers or radio transmitter, 
% then transmitted in the air channel or telephony network 
% and finally recorded by microphones.
% % Compared to over-the-line, they are lossy medium and the produced voices is at the risk of losing effectiveness.
% Compared to over-the-line, they are lossy medium due to noises from many aspects, thus may destroy the effectiveness of produced voices.
% In this work, we only consider over-the-line and over-the-air physical attacks.
Depending on the scenario, adversarial voices can be passed to SR models over different mediums, 
% including over-the-line and over-the-air. 
including API and air channel. 
% Over-the-line attack 
API attack 
directly feeds adversarial voices in the form of audio file to models 
% via exposed API, 
via models' exposed interface, 
thus it will not introduce any disruption to adversarial voices.
In contrast, over-the-air attack, where adversarial voices are played/recorded by loudspeakers/microphones 
and transmitted in the air channel, 
is a lossy procedure.
% Adversarial voices will lose effectiveness with high probability due to distortion caused by over-the-air attack.
% Adversarial voices will lose effectiveness with high probability due to distortion occurred in this procedure.
The distortion occurred in this procedure will cause adversarial voices to lose effectiveness with high probability.
Over-the-air attack is generally more practical and realistic yet more challenging 
% than over-the-line attack. 
than API attack. 


In this section, we first present the acoustic model of over-the-air attack.
This model helps us understand the factors affecting the effectiveness of adversarial voices under over-the-air condition.
% Then, we recap four techniques utilized to build robust adversarial voices 
% which can survive from over-the-air transmission in the physical world.
Then, we recap four techniques toward practical adversarial voices 
which can survive from over-the-air transmission in the physical world.
% toward practical audio adversarial examples which could remain
% effective while being played over the air in the physical world

\subsubsection{Acoustic Model for Over-the-air Attack}
\figurename~\ref{fig:over-the-air-model} illustrates the acoustic model for over-the-air attack. 
When an adversary initializes over-the-air adversarial attack, 
the voice is first emitted by a loudspeaker, then propagated in the air channel, and finally recorded by the victim' microphone. 
Overall, when travelling through the air, an adversarial voice $x^{adv}$ inevitably experiences three types of distortion: 
equipment distortion, ambient noise and reverberation.

\smallskip\noindent {\bf Equipment distortion.}
Equipment distortion is introduced by loudspeakers and microphones due to their frequency-selectivity feature.
Specifically, their frequency response is non-uniform across the frequency band 
with amplification in some frequency ranges and attenuation in others.
This will distort the transmitted voices and undermine the attack.
Roughly speaking, different brands of loudspeakers and microphones exhibit different frequency responses, 
thus incurring different levels of distortion to adversarial voices.
% The impact of equipment distortion on adversarial voices can also be measured in the time domain 
% via loudspeakers and microphones' impulse response $h$.
We can also measure the impact of equipment distortion on adversarial voices in the time domain 
via loudspeakers and microphones' impulse response $h$.
The adversarial voice disrupted by equipment distortion is formulated as $x^{adv}\otimes h$ where $\otimes$ denotes convolution operation.
% impule response
% frequency selected

\smallskip\noindent {\bf Ambient noise.}
In practice, ambient noise is inevitable in playback and recording environment.
It includes various types of noise, including ambient human voice, background music, traffic noise and so on, 
% depending on the specific scenario where the attack is launched (e.g., living room, office, airport, and mall).
depending on the specific attack scenario (e.g., living room, office, airport, and mall).
These noises, denoted by $n$, influence the effectiveness of adversarial voices by additively changing their magnitude, 
i.e., from $x^{adv}$ to $x^{adv}+n$.
% However, the influence varies with the relative intensity of ambient noise to adversarial voices, i.e., Signal-to-Noise Ratio (SNR).
However, the influence varies with the relative strength of ambient noise to adversarial voices, 
i.e., Signal-to-Noise Ratio (SNR) between adversarial voices and ambient noise.
Ambient noise with low volume has limited impact since weak noises are easily overwhelmed by stronger voices~\cite{Metamorph}, and vice versa.

\smallskip\noindent {\bf Reverberation.}
When played by loudspeakers in indoor environment, 
% an adversarial voice will propagate through multiple paths (i.e., direct path and other reflected paths) with various delays and attenuation.
a voice signal will propagate through multiple paths (i.e., direct path and other reflected paths) 
with various delays and absorption by many surfaces.
When the direct sound and reflections blend and overlap with each other, reverberation is created.
Reverberation will cause the received voice by microphones to be largely different from the original voice sent out by loudspeakers.
% Room Impulse Response (RIR) can be utilized to characterize the transfer function from the original voice to the received voice.
% Room Impulse Response (RIR), represented by $r$, can reproduce reverberation in the captured environment by convolving it with $x^{adv}$ 
% to create the adversarial voice with reverberation $x^{adv}\otimes r$.
Room Impulse Response (RIR), represented by $r$, can well characterize the acoustic properties 
of a room regarding sound propagation and reflections.
The adversarial voice with reverberation is created by convolving $r$ with $x^{adv}$, i.e., $x^{adv}\otimes r$.
RIR varies with the room configuration (e.g., room dimension, reverberation time and absorption coefficient of reflective materials) 
as well as the location of loudspeakers and microphones.
% RIR can be obtained by either simulation or real-world measurement.
% Simulation leverages Image Source Method~\cite{image-method} 
To obtain RIR for a specific room, two different methods are mostly used in practice: simulative approach and real-world measurement.
Simulative approach leverages the well-known Image Source Method~\cite{image-method}
which accepts room configuration and hardware's position as input and returns the simulated RIR.
As for real-world measurement, we can transmit a brief input signal (called impulse) by a loudspeaker in a room, 
then the response signal recorded by a microphone is the RIR of this room under the current position of loudspeaker and microphone. 
However, as the impulse signal also goes through the hardware during transmission, 
the RIR obtained by real-world measurement is indeed the composite impulse response of the room and hardware~\cite{Metamorph,hang-practical}, i.e., $r\circ h$.

\subsubsection{Robust Adversarial Voices}
To enhance the robustness of adversarial voices and enable physical over-the-air attack, 
previous works either integrate the effect of aforementioned distortions into the 
generation process of adversarial voices~\cite{yuan2018commandersong,ijcai2019-741,qin2019imperceptible,Metamorph,hang-practical,xie2021real,xie-universal,LiW00020} 
by redesigning the loss function, 
or simply craft adversarial voices with high-confidence~\cite{chen2019real}.

\smallskip\noindent {\bf Band Pass Filter.}
To mitigate the effect of equipment distortion introduced by hardware's frequency-selectivity, 
% \cite{ijcai2019-741,LiW00020} introduced a band-pass filter, which can explicitly limit adversarial perturbations 
% to be in the valid frequency range (i.e., the frequency range without too much attenuation), into the loss function. 
% \cite{ijcai2019-741,LiW00020} introduced a band-pass filter into the loss function, 
% which can explicitly limit adversarial perturbations to be in the valid frequency range, 
% i.e., the frequency range where there is no clear attenuation in the hardware frequency response.
\cite{ijcai2019-741,LiW00020} introduced a band-pass filter into the loss function, 
which can explicitly limit adversarial perturbations to be in the frequency range 
where there is no clear attenuation in the hardware frequency response.
% The loss function is modified to $L(f(x+{\tt BPF}(\delta)), y)$ 
The loss function is modified to $f(x+{\tt BPF}(\delta),y)$ 
% such that the crafted adversarial voices will acquire robustness such that they function even
% when frequency bands outside the audible range are cut by a speaker or a microphone.
such that the crafted adversarial voices will acquire robustness against hardware's frequency-selectivity.

\smallskip\noindent {\bf Random Noise.}
\cite{yuan2018commandersong}, \cite{ijcai2019-741} and \cite{LiW00020} 
use uniform noise, white Gaussian noise and isotropic noise to emulate the impact of ambient noise in the physical attack scenario, 
and incorporate them into the loss function, i.e., 
% $\mathbb{E}_{n\sim \mathcal{N}} L(f(x+\delta+n), y)$ 
$\mathbb{E}_{n\sim \mathcal{N}} f(x+\delta+n,y)$ 
where $\mathcal{N}$ denotes the distribution of random noise. 

\smallskip\noindent {\bf Room Impulse Response.}
% \cite{ijcai2019-741,qin2019imperceptible,LiW00020,hang-practical,xie2021real,xie-universal,Metamorph} introduce RIR into the generation of 
% adversarial voices by modifying the loss function as $\mathbb{E}_{r\sim } f(r(t) * x^{adv})$. 
To improve the robustness of adversarial voices against reverberation in physical recording environment, 
\cite{ijcai2019-741,qin2019imperceptible,LiW00020,hang-practical,xie2021real,xie-universal,Metamorph} 
reproduce reverberation in the generation procedure by pre-coding RIR into the loss function, i.e., 
% $L(f(r\otimes (x+\delta)), y)$. 
$f(r\otimes (x+\delta), y)$. 
Since RIR varies largely depending on room configurations and devices' locations, 
instead of using a single RIR, 
some works~\cite{ijcai2019-741,qin2019imperceptible,LiW00020,xie2021real,xie-universal,Metamorph} 
use a set of RIR $\mathcal{R}$ collected in diverse environments. 
The loss function becomes 
% $\mathbb{E}_{r\sim \mathcal{R}} L(f(r \otimes (x+\delta)), y)$.
$\mathbb{E}_{r\sim \mathcal{R}} f(r \otimes (x+\delta), y)$.
In this way, it is expected that the obtained adversarial voices can work in various launching condition and environments 
and attack numerous victim devices simultaneously.
% modifying the loss function as $\mathbb{E}_{r\sim } f(r(t) * x^{adv})$. 
% By minimizing this loss function, the crafted adversarial will remain effective when played in the room.

\smallskip\noindent {\bf Improving Confidence.}
% \cite{chen2019real} argued that the above methods are device and environment dependent to some extent.
% To address this, \cite{chen2019real} proposed to improve the confidence of the adversarial voices.
% This will push the crafted adversarial voices far from the decision boundary, thus they become resilient against the noise.
\cite{chen2019real} argued that the high sensitivity of adversarial voices to the distortion incurred by over-the-air propagation 
is attributed to their closeness from decision boundary.
Motivated by this, the authors address the challenge of launching practical attack over the air 
by generating high-confidence adversarial examples.
They experimentally show that their approach produces adversarial examples with enough resilience against over-the-air distortion, 
and is device/environment-independent to some extent.

\begin{figure}
    \includegraphics[width=0.48\textwidth]{fig/over-the-air}
    \caption{The acoustic model of over-the-air attack.}
    \label{fig:over-the-air-model}
\end{figure}


==> background.tex <==

\section{Background}\label{sec:background}
In this section, we provide an overview of speaker recognition systems and introduce the threat model of our attack.

\subsection{Speaker Recognition Systems}\label{sec:SRSs}

In this subsection, we introduce the preliminaries of mainstream and cutting-edge SRSs as well as their recognition tasks.

% \vspace*{-1mm}\subsection{Overview of Speaker Recognition}\vspace*{-1mm}
\smallskip\noindent {\bf Overview of Speaker Recognition.}
Modern and cutting-edge SR represent characteristics of speakers as fixed-dimensional vectors, 
i.e., speaker embedding~\cite{wang2020simulation}.
\figurename~\ref{fig:typical-SRSs} depicts a generic architecture of embedding-based SRSs, 
which includes three stages: training, enrollment, and recognition.
In the training stage, tens of thousands of voices from thousands of training speakers are utilized to train a background model.
The background model will learn the mapping from voices to embeddings in the vector space.
Conventional background model is based on the Gaussian Mixture Model (GMM)~\cite{ReynoldsR95,reynolds2000speaker}, 
and produces identity-vector (ivector)~\cite{DehakDKBOD09} as embeddings.
Recent state-of-the-art background model is based on deep neural networks, 
and outputs deep embeddings, e.g., dvector~\cite{variani2014deep} or xvector~\cite{snyder2018x}.
%
In the enrollment stage, the background model maps each enrolling speaker's voice to an \emph{enrollment embedding},
which is regarded as the unique identity of the enrolling speaker.
%
In the recognition stage, given a voice of an unknown speaker, the \emph{voice embedding} is retrieved from the background model
for scoring. The scoring module computes the similarity between the \emph{enrollment embedding} 
and \emph{voice embedding} based on which the result is produced by the decision module.
There are two widely-used scoring approaches: Probabilistic Linear Discriminant Analysis (PLDA)~\cite{nandwana2019analysis}
and COSine Similarity (COSS)~\cite{dehak2010cosine}.
% The former approach works well in most situations, but needs to be trained using the extracted embeddings of training voices from the background model~\cite{wang2020simulation}.
The former approach works well in most situations, but needs to be trained using the embeddings of training voices~\cite{wang2020simulation}.
The latter approach is a reasonable substitution of PLDA which does not need to be trained.
% The decision module, denoted by $D()$

The acoustic feature extraction module converts raw speech signals to acoustic features
carrying characteristics of the raw signals.
Common feature extraction algorithms include speech spectrogram~\cite{hannun2014deep}\cite{amodei2016deep}, 
Filter-bank~\cite{FilterBanks}\cite{li2017deep}, MFCC~\cite{muda2010voice}, and PLP~\cite{hermansky1990perceptual}.
Note that some neural network-based SRSs do not rely on acoustic feature extraction 
since they accept raw waveforms as input, e.g., SincNet~\cite{SincNet}.
Their feature extraction is left to be handled by the internal neurons of neural networks.

\begin{figure}
    \includegraphics[width=0.48\textwidth]{fig/SRSs-2}
    % \caption{The overview of speaker recognition.}
    \caption{A generic architecture of embedding-based speaker recognition.}
    \label{fig:typical-SRSs}
\end{figure}

% \vspace*{-2mm}\subsection{Sub-tasks of Speaker Recognition}\label{sec:SR-task}\vspace*{-1mm}
% \vspace*{-2mm}\subsection{Recognition Tasks of Speaker Recognition}\label{sec:SR-task}\vspace*{-1mm}
\smallskip\noindent{\bf Recognition Tasks of Speaker Recognition.}
% Speaker recognition can be divided into three sub-tasks: open-set identification (OSI), 
Speaker recognition can be divided into three tasks: open-set identification (OSI), 
close-set speaker identification (CSI) and speaker verification (SV).
OSI allows multiple speakers
to be enrolled during the enrollment stage,
forming a speaker group $G$.
For an arbitrary input voice $x$, the system determines whether $x$ is uttered by one of the enrolled speakers
or none of them, according to the scores of all the enrolled speakers and a preset (score) threshold $\theta$.
Formally, suppose the speaker group $G$ has $n$ speakers $\{1,2,\cdots,n\}$,
the decision module outputs $D(x)$: % for an input voice $x$ as follows:
% \begin{center}
% $D(x)=\left\{
% \begin{array}{ll}
% \arg\max\limits_{i\in G} \ [S(x)]_i, &\mbox{if } \max\limits_{i\in G} \ [S(x)]_i\geq \theta; \\
% {\tt reject}, &\mbox{otherwise}.
% \end{array}\right.$
% \end{center}
\begin{center}
    $D(x)=\left\{
    \begin{array}{ll}
    \arg\max\limits_{i\in G} \ [S(x)]_i, &\mbox{if } \max\limits_{i\in G} \ [S(x)]_i\geq \theta; \\
    % {\tt reject}, &\mbox{otherwise}.
    {\tt imposters}, &\mbox{otherwise}.
    \end{array}\right.$
    \end{center}
where $[S(x)]_i$ for $i\in G$ denotes the score of the voice $x$ that is uttered by the speaker $i$.
Intuitively, the system classifies the input voice $x$ as the speaker $i$ 
if and only if the score $[S(x)]_i$ of the speaker $i$ is the largest one among all the enrolled speakers, 
and not less than the threshold $\theta$.
If the largest score is less than $\theta$, the system directly rejects the voice, namely,
it is not uttered by any of the enrolled speakers. 

CSI and SV systems accomplish similar tasks as the OSI system, but with some special settings.
A CSI system never rejects any input voices, i.e., an input will always be classified as one of the enrolled speakers.
Whereas an SV system can have exactly \emph{one} enrolled speaker
and checks if an input voice is uttered by the enrolled speaker. 
% i.e., either \emph{accept} or \emph{reject}.
% Note that in some works~\cite{du2020sirenattack,jati2021adversarial,DBLP:journals/corr/abs-1711-03280}, 
% CSI also refers to the task where the enrollment stage is not involved, 
% and the background model is directly utilized to identify the training speakers.
% To discriminate the difference, we further classify CSI into two sub-tasks: 
% CSI with enrollment (CSI-E) and CSI without enrollment (CSI-NE).
% Ideally, a recognized speaker in CSI-NE task is involved in the training stage, 
% while a recognized speaker in CSI-E task should have enrolled in the enrollment stage but may not be involved in the training stage.

\subsection{Threat Model}\label{sec:threat-model}
\chengk{I am writing this part.}

% In this subsection, we precisely define the threat model in this work, including the adversary's goals, capabilities and knowledge, 
% following the recommendation for describing threat model in \cite{evaluate-robustness}.

We assume that the adversary intends to craft an adversarial example from a voice uttered by some source speaker, 
so that it is classified as one of the enrolled speakers (untargeted attack)
or the target speaker (targeted attack) by the SRS under attack,
but is still recognized as the source speaker by ordinary users. 

As shown in \tablename~\ref{tab:goal}, the adversary may attempt to achieve various goals in performing such attack, 
including malicious goals, e.g., unauthorized access, Denial-of-Service (Dos), anonymous access, and evasion, 
and beneficial goals, e.g., privacy protection. 

The adversary carefully choose the source and/or target speakers involved in the attack to achieve his motivation. 
Another factor influencing the adversary's choice of source speaker is his capacity, 
i.e., the set of voices that are available to the adversary. 
Generally, it is trivial for the adversary to obtain voices uttered by the speakers out of the enrolled speaker group $G$, 
considering the large amount of audio medias available online and open-source speech datasets. 
As for the voices uttered by the enrolled speakers, 
the adversary may have none of them, or can access to them by privately collecting them in advance. 
When the adversary has two options, 
he may choose an imposter as the source speaker to avoid altering the awareness of a third-party person 
who is familiar with all the enrolled speakers, 
or one of the enrolled speaker to save the attack cost (cf. section~\ref{sec:evaluation}). 
In conclusion, the goal and the capacity of the adversary decides the selection of source and/or target speakers, 
as shown in \figurename~\ref{fig:attack-overview}.




% \smallskip\noindent {\bf Adversary's Goal.}
% An adversary can achieve different goals of crafting adversarial examples 
% by using benign voices with different ground-truths 
% and launching untargeted/targeted attacks on different recognition tasks.
% \chengk{To DO: goal}
% % In this work, we focus on the goal of causing untargeted misclassification to the CSI SR model, that is, given a benign voice $x$ with ground-truth $y\in\{1,2,\cdots,M\}$, crafting an adversarial voice $x^{adv}$ such that ${\tt SR}_{\text{CSI}}(x^{adv})\neq y$.
% % We highlight two practically feasible attack scenarios associated with this goal:
% % (1) the adversary crafts adversarial voices for the super user of smart home who has exclusive control over some devices. These voices are wrongly recognized as arbitrary ordinary users, causing Denial-of-Service (DoS) to the super user.
% % (2) the criminal manipulates his voices to render the voiceprint-based criminal detection system to recognize him as arbitrary legitimate citizens.

% \smallskip\noindent {\bf Adversary's Capabilities.}
% Apart from deceiving SR models, adversarial perturbation are required to be imperceptible to human hearings. 
% Thus, the adversary is not permitted to arbitrarily manipulate the perturbation. 
% In this work, we adopt $L_\infty$ norm to quantify the magnitude of the perturbation 
% and set an upper bound for this norm, 
% the same as large bodies of works~\cite{DBLP:journals/corr/abs-1711-03280, abs-1801-03339, 
% li2020adversarial,jati2021adversarial, zhang2021attack,chen2019real}.
% The adversary is only allowed to add a small perturbation which does not exceed this upper bound to benign voices.
% % We also assume that the adversary can launch digital domain attack, 
% % i.e., feeding crafted adversarial voices in the form of audio file to the SR models directly via exposed API. 
% % Over-the-air attack, where the adversarial voices are played by loud speakers, 
% % then transmitted in the air channel and finally recorded by microphones, is out of the scope of this work.
% % Under digital domain attack, the adversary does not need to take into account ambient and hardware noises 
% % accrued in over-the-air attack which would destroy the effectiveness of adversarial voices.
% % This assumption is practical and realistic given that commercial SRSs 
% % (e.g., Microsoft Azure~\cite{microsoft-azure-vpr} and SpeakIn~\cite{SpeakIn}) 
% % provide their API to the public to access their services.

% \smallskip\noindent {\bf Adversary's Knowledge.}
An adversary may own different levels of knowledge about the SR model under attack, 
from white-box access to model structure and parameters, 
to black-box access to model outputs (decisions and/or scores).
% Based on different knowledge about SR models, we take into account three attack scenarios: 
% white-box attack, query-based attack and transfer-based attack.
% White-box attack relies on detailed information of the victim model, 
% including internal architecture and learned parameters values.
% Thus, a white-box attack adversary can easily and precisely computes 
% the gradient of the loss w.r.t. the input by backpropagation.
% On the contrary, black-box attack, including query-based and transfer-based attacks, 
% assumes no knowledge about the model 
% since the model is not transparently exposed to adversaries. 
% Despite this, query-based attack can access the target model as an oracle, i.e., 
% providing a series of carefully crafted inputs to the model and observing its outputs.
% Transfer-based attack is based on adversarial transferability 
% that adversarial examples crafted on one model remain effective for others. 
% It is more practical in real-world applications yet more challenging 
% since it cannot utilize the adaptive queries as in query-based attack. 
Note that under white-box, we assume the adversary can access to the speaker model with enrolled speakers, not the background model. 
This knowledge restricts the optimization approach (white-/black-box approaches) the adversary can adopt in our attack \attackname, 
as shown in \figurename~\ref{fig:attack-overview}.

Additionally, the adversary may or may not own knowledge about the real-world environment where the attack would be launched.
% Another kind of knowledge is the knowledge about the attack environments where the attack would be launched. 
A sophisticated adversary may anticipate its layout (e.g., room dimension and the kind of reflective materials), 
collect in advance reverberation impulse response and ambient noise dedicated for that environment, 
or acquire the property of the victim's devices. 
As such, as shown in \figurename~\ref{fig:attack-overview}, he can use specific and customized transformation functions during the construction of adversarial voices instead of generic ones, 
and the crafted adversarial voices are expected to work more robustly in that environment.

% \begin{table}[t]
%     \begin{tabular}{}
        
%     \end{tabular}
% \end{table}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{fig/overview-attack-2}
    \caption{The overview of our attack \attackname.}
    \label{fig:attack-overview}
\end{figure*}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{fig/overview-attack}
%     \caption{The overview of our attack \attackname.}
%     \label{fig:attack-overview}
% \end{figure}
\begin{table*}[htbp]
    \centering
    \caption{Add caption}
    \resizebox{1.0\textwidth}{!}{%
      \begin{tabular}{|c|c|c|c|c|}
      \toprule
      \multicolumn{3}{|c|}{\textbf{Goal}} & \textbf{Source Speaker} & \textbf{Target Speaker} \\
      \midrule
      \multirow{10}[20]{*}{\textbf{Malicious}} & \multirow{3}[6]{*}{\bf Unauthorized Access} & \multirow{2}[2]{*}{obtain the privilege exclusive to $G_1\subset G$} & $s\in G\setminus G_1$ & $t\in G_1$ \\
  \cmidrule{4-5}          &       &       & $s\notin G$ & $t\in G_1$ \\
  \cmidrule{3-5}          &       & obtain the common privilege shared by $G$ & $s\notin G$ & Untargeted \\
  \cmidrule{2-5}          & \multirow{3}[6]{*}{\bf Denial-of-Service} & hinder speaker $s$ from accessing common services shared by $G$  & $s\in G$ & $t\notin G$ \\
  \cmidrule{3-5}          &       & \multirow{2}[2]{*}{hinder speaker $s$ from accessing his exclusive services  } & $s\in G$ & $t\notin G$ \\
  \cmidrule{4-5}          &       &       & $s\in G$ & Untargeted \\
  \cmidrule{2-5}          & \multirow{2}[4]{*}{\bf Anonymous Access} & speaker $s$ hides his identity when accessing illegal services & $s\in G$ & Untargeted \\
  \cmidrule{3-5}          &       & also cause reputation degrade to a specific speaker  & $s\in G$ & $t\in G\setminus\{s\}$ \\
  \cmidrule{2-5}          & \multirow{2}[4]{*}{\bf Evasion} & anomalous subject $s$ evades detection (single anomalous subject) & $s\in G$ & Untargeted \\
  \cmidrule{3-5}          &       & anomalous subject $s$ evades detection (multiple anomalous subjects $G_2\subset G$) & $s\in G$ & $t\in G\setminus G_2$ \\
      \midrule
      \textbf{Beneficial} & {\bf Privacy Protection} & protect privacy against excessive surveillance & $s\in G$ & Untargeted \\
      \bottomrule
      \end{tabular}%
    }
    \label{tab:goal}%
  \end{table*}%
  

==> discussion.tex <==

\section{Discussion}\label{sec:discussion}
\chengk{To be moved to conclusion.}

%\sen{Stopped}
% To shed further light on the research direction in this field,
% in this section, we discuss the limitations of our study, 
% % more threatening attacks, and more rigorous understanding of attacks as well as defenses 
% more threatening attacks, and more rigorous understanding of attacks  
% in the speaker recognition domain.
In this section, we discuss the limitations of our study and 
more threatening attacks in the speaker recognition domain, to shed further light on the research direction in this field.

\subsection{Limitations}

\subsubsection{Suitability of $L_p$ norm, SNR, and PESQ as stealthiness metrics}
In this work, we use $L_\infty$ and $L_2$ norms to measure the perturbation magnitude during the procedure of constructing adversarial example,
and utilize $L_2$ norm, SNR, and PESQ to measure the stealthiness of crafted adversarial voices.
These metrics have been widely adopted in the literatures~\cite{chen2019real,du2020sirenattack,jati2021adversarial,LiZJXZWM020,shamsabadi2021foolhd,WangGX20,zhang2021attack}
and in general, can consistently reflect the degree of distortions according to our experimental results.
Moreover, PESQ is an objective perceptual measure simulating the human auditory system~\cite{xiang2017digital}.
However, it remains unknown to what extent do these metrics correlate with human hearing perception.
% In image domain, \cite{suitibility-lp} showed that proximity of two images measured by $L_p$ norm is neither sufficient nor necessary for them to be perceptually similar.
In the image domain, the proximity of two images measured by $L_p$ norm is neither necessary nor sufficient for them to be visually indistinguishable by humans~\cite{suitibility-lp}.
Therefore,  it is worthy to explore in future the sufficiency and necessity of these metrics in quantifying
% audibly indistinguishable by humans.
the audio perceptual similarity.

\subsubsection{The best loss function for transfer attack}
Throughout our transferability analysis in Section~\ref{sec:transfer-analysis}, 
we utilize the best loss functions empirically identified in section~\ref{sec:evaluation} 
for each case of source and target speakers. 
However, since the evaluation in Section~\ref{sec:evaluation} targets ordinary non-transfer attacks, 
the attack with the best identified loss functions do not necessarily lead to the most transferable adversarial examples. 
As shown in the recent work~\cite{simple-transfer} about transfer attack in image domain, 
% some loss functions achieve higher transferability success rate than other loss functions. 
some loss functions largely outperform other loss functions in terms of transferability success rate. 
The superiority becomes more obvious under challenging transfer scenarios, 
such as the source and target models have different architectures, 
and the targeted label is specified as the lowest-ranked/least-likely class (i.e., Targeted Least Likely). 
Therefore, exploring the best loss function which yields the best transferability success rate 
for each case of source and target speakers is a worthwhile future work. 

\subsubsection{Explaining and understanding transferability}
We have empirically demonstrated that adversarial voices generated for one SR model do transfer to other models, 
but theoretically explaining why adversarial examples transfer remains a question. 
Previous work~\cite{Space-Adver} and \cite{Delving-Transfer} suggest that the similarity of decision boundaries 
learned by the source and target models enable the transfer of adversarial examples. 
However, as shown in Section~\ref{sec:transfer-model}, the transferability is non-symmetric, i.e., 
adversarial voices generated from SR model {\it X} transfer to model {\it Y} easily 
does not mean the opposite is also natural. 
This phenomenon challenges the explanation based on decision boundaries similarity 
since similarity is a systematical metric. 
% It remains as a feature work to provide more suitable analysis and explanation. 
Providing explanation and understanding consistent with this phenomenon is an important follow-up work. 

% \subsection{More Threatening Attacks}
% \sen{It is uncertain whether this section should be provided for a journal paper.}

% % \subsubsection{Double source or target universal perturbation}
% % \subsubsection{Multiple source or target universal perturbation}
% % \subsubsection{Multiple target universal perturbation}
% \subsubsection{Arbitrary source-to-target universal perturbation}
% By adopting appropriate loss functions, 
% our attack \attackname can be exploited to launch adversarial attack with arbitrary source and target speakers. 
% Despite its powerful capability, it is input-specific, 
% i.e., for each voice uttered by the selected source speaker, 
% the adversary needs to craft a perturbation from scratch designated for the voice. 
% In the future, we will strengthen our attack by creating universal perturbation~\cite{Universal-Survey}. 
% A universal adversarial perturbation is a single perturbation which is capable to 
% deceive a model when being added to most benign examples. 
% As such, it is expected that our attack can construct voice-agnostic adversarial perturbation 
% with arbitrary source and target speakers.  


% \subsubsection{More transferable adversarial examples}
% As shown in \tablename~\ref{tab:transfer-OSI}, \tablename~\ref{tab:transfer-CSI-Untargeted}, 
% \tablename~\ref{tab:transfer-CSI-targeted}, and \tablename~\ref{tab:transfer-SV}, 
% transfer attack is remarkably difficult when the model similarity between the source and target models is low, 
% especially for targeted transfer attack. 
% Though challenging, transfer attack is much more practical than whit-box and query-based black-box attack 
% since it neither assumes any prior knowledge about the victim model nor repeatedly interacting with it.  
% Therefore, improving the capacity of transfer attack towards more transferable adversarial voices is an important follow-up work. 
% One possible solution is advanced gradient descent. 
% While plain gradient descent only focus on current gradients at each iteration and overlook previous gradients, 
% \cite{Momentum} integrates a momentum term to accumulate previous gradients and achieve more stable update directions. 
% Similarly, \cite{Nesterov} instead exploits Nesterov accelerated gradient, a more advanced technique than momentum-based gradient. 
% \cite{Variance-Tuning} achieves the same goal by reducing the variance of gradient 
% via averaging the gradients of multiple examples corrupted by uniform noise. 
% These techniques help the attack escape from poor local optima 
% and have been shown to yield more transferable adversarial examples in the image domain. 
% Validating their effectiveness in speaker recognition domain is a worthwhile future work. 



% % \subsection{More Rigorous Understanding of Attacks and Defenses}
% \subsection{More Rigorous Understanding of Attacks}

% \subsubsection{Explaining and understanding transferability}
% We have experimentally demonstrated that adversarial voices generated for one SR model do transfer to other models, 
% although the transferability rate varies with the pair of source and target models. 
% % An interesting question is why adversarial examples transfer and why the transferability rate varies. 
% Despite this, it remains a question why adversarial examples transfer. 
% Previous work~\cite{Space-Adver} and \cite{Delving-Transfer} suggest that the similarity of decision boundaries 
% learned by the source and target models enable the transfer of adversarial examples. 
% However, as shown in section~\ref{sec:transfer-model}, the transferability is non-symmetric, i.e., 
% adversarial voices generated from SR model {\it X} transfer to model {\it Y} easily 
% does not mean the opposite is also natural. 
% This phenomenon challenges the explanation based on decision boundaries similarity 
% since similarity is a systematical metric. 
% % It remains as a feature work to provide more suitable analysis and explanation. 
% Providing explanation and understanding consistent with this phenomenon is an important follow-up work. 

% \subsubsection{Re-evaluation of more defenses}


==> note.tex <==

\noindent Decision module $D(x):\mathbb{R}^{*}\rightarrow \mathcal{D}$; Scoring module $S(x): \mathbb{R}^{*}\rightarrow \mathbb{R}^{*}$

\noindent Equation in \textcolor{red}{red} is covered and experimentally demonstrated in FAKEBOB~\cite{chen2019real}.

\noindent Equation in \textcolor{blue}{blue} is covered in FAKEBOB, but no experiment.

\noindent Equation in \textcolor{black}{black} is not covered in FAKEBOB.

\noindent CSI: $\mathcal{\mathcal{D}}=\{1,2,\cdots,n\}(n>1)$
% {\small
\begin{align}
\begin{cases}
	m\in \mathcal{D} & 
	\begin{cases} 
		\text{untar *} & \color{blue} f_{\text{M}}^{1}(x)=[S(x)]_m-{\tt max}_{i\in \mathcal{D},i\neq m}[S(x)]_i +\kappa \\ 
		% \text{target} & f(x)={\tt max}_{i\in \mathcal{D},i\neq t}[S(x)]_i - [S(x)]_t + \kappa\ (t\in \mathcal{D}, t\neq m)
        \text{target *} & \color{red} f_{\text{M}}^{2}(x)={\tt max}_{i\in \mathcal{D},i\neq t}[S(x)]_i - [S(x)]_t + \kappa\ (t\in \mathcal{D})
	\end{cases} \\
	m=-1 & 
	\begin{cases} 
		\text{untar} & \text{no sense} \\ 
		% \text{target} & f(x)={\tt max}_{i\in \mathcal{D},i\neq t}[S(x)]_i - [S(x)]_t + \kappa\ (t\in \mathcal{D}, t\neq D(x))
        \text{target *} & \color{blue} f_{\text{M}}^{2}(x)={\tt max}_{i\in \mathcal{D},i\neq t}[S(x)]_i - [S(x)]_t + \kappa\ (t\in \mathcal{D})
	\end{cases}
\end{cases}
\end{align}
% }

\noindent SV: $\mathcal{D}=\{-1, 1\}$ $-1: {\tt reject}\ 1: {\tt accept}$
% {\small
\begin{align}
\begin{cases}
	m=1 & f_{\text{M}}^{3}(x) = S(x)-\theta+\kappa \\
	m=-1 & \color{red} f_{\text{M}}^{4}(x) = \theta - S(x) + \kappa
\end{cases}
\end{align}
% }

\noindent OSI: $\mathcal{D}=\{-1, 1,2,\cdots,n\}(n>1)$  $-1: {\tt reject}$
% {\small
\begin{align}
    \begin{cases}
        m\in \mathcal{D}\setminus\{-1\} & 
        \begin{cases} 
            \text{untar *} & f(x)={\tt min}\{f_{\text{M}}^{5}={\tt max}_{i\in \mathcal{D}\setminus\{-1\}}[S(x)]_i-\theta+\kappa,\ f_{\text{M}}^{6}={\tt max}\{\theta, [S(x)]_m\}-{\tt max}_{i\in \mathcal{D}\setminus\{-1\},i\neq m}[S(x)]_i +\kappa\} \\ 
            \text{target} & 
            \begin{cases}
                * t\in \mathcal{D}\setminus\{-1\},t\neq m & f_{\text{M}}^{7}(x)={\tt max}\{\theta, {\tt max}_{i\in \mathcal{D}\setminus\{-1\},i\neq t}[S(x)]_i\} - [S(x)]_t + \kappa \\
                t=-1 & f_{\text{M}}^{5}(x)= {\tt max}_{i\in \mathcal{D}\setminus\{-1\}}[S(x)]_i-\theta+\kappa
            \end{cases}
        \end{cases} \\
        m=-1 & 
        \begin{cases} 
            \text{untar} & \color{blue} f_{\text{M}}^{8}(x)=\theta - {\tt max}_{i\in \mathcal{D}\setminus\{-1\}}[S(x)]_i +\kappa \\ 
            \text{target *} & \color{red} f_{\text{M}}^{7}(x)={\tt max}\{\theta, {\tt max}_{i\in \mathcal{D}\setminus\{-1\},i\neq t}[S(x)]_i\} - [S(x)]_t + \kappa\ (t\in \mathcal{D}\setminus\{-1\})
        \end{cases}
    \end{cases}
    \end{align}

    Margin-NO-2: $f_{\text{M}}^{9}(x)=\theta-[S(x)]_t+\kappa$ (target)\ $f_{\tt min}^{5, 10}={\tt min}\{f_{\text{M}}^{5}(x), f_{\text{M}}^{10}(x)=\theta-{\tt max}_{i\in \mathcal{D}\setminus\{-1\},i\neq m}[S(x)]_i+\kappa\}$ (untarget)
    
    Margin-NO-T: $f_{\text{M}}^{2}(x)$ (target) \quad $f_{\tt min}^{5, 1}={\tt min}\{f_{\text{M}}^{5}(x), f_{\text{M}}^{1}(x)\}$ (untarget)
    % }

==> threat-model.tex <==
\section{Threat Model}\label{sec:threat-model}
In this section, we precisely define the threat model in this work, including the adversary's goals, capabilities and knowledge, 
following the recommendation for describing threat model in \cite{evaluate-robustness}.

\smallskip\noindent {\bf Adversary's Goal.}
An adversary can achieve different goals of crafting adversarial examples 
by using benign voices with different ground-truths 
and launching untargeted/targeted attacks on different recognition tasks.
\chengk{To DO: goal}
% In this work, we focus on the goal of causing untargeted misclassification to the CSI SR model, that is, given a benign voice $x$ with ground-truth $y\in\{1,2,\cdots,M\}$, crafting an adversarial voice $x^{adv}$ such that ${\tt SR}_{\text{CSI}}(x^{adv})\neq y$.
% We highlight two practically feasible attack scenarios associated with this goal:
% (1) the adversary crafts adversarial voices for the super user of smart home who has exclusive control over some devices. These voices are wrongly recognized as arbitrary ordinary users, causing Denial-of-Service (DoS) to the super user.
% (2) the criminal manipulates his voices to render the voiceprint-based criminal detection system to recognize him as arbitrary legitimate citizens.

\smallskip\noindent {\bf Adversary's Capabilities.}
Apart from deceiving SR models, adversarial perturbation are required to be imperceptible to human hearings. 
Thus, the adversary is not permitted to arbitrarily manipulate the perturbation. 
In this work, we adopt $L_\infty$ norm to quantify the magnitude of the perturbation 
and set an upper bound for this norm, 
the same as large bodies of works~\cite{DBLP:journals/corr/abs-1711-03280, abs-1801-03339, 
li2020adversarial,jati2021adversarial, zhang2021attack,chen2019real}.
The adversary is only allowed to add a small perturbation which does not exceed this upper bound to benign voices.
% We also assume that the adversary can launch digital domain attack, 
% i.e., feeding crafted adversarial voices in the form of audio file to the SR models directly via exposed API. 
% Over-the-air attack, where the adversarial voices are played by loud speakers, 
% then transmitted in the air channel and finally recorded by microphones, is out of the scope of this work.
% Under digital domain attack, the adversary does not need to take into account ambient and hardware noises 
% accrued in over-the-air attack which would destroy the effectiveness of adversarial voices.
% This assumption is practical and realistic given that commercial SRSs 
% (e.g., Microsoft Azure~\cite{microsoft-azure-vpr} and SpeakIn~\cite{SpeakIn}) 
% provide their API to the public to access their services.

\smallskip\noindent {\bf Adversary's Knowledge.}
An adversary may own different levels of knowledge about the SR model under attack, 
from white-box access to model structure and parameters, 
to black-box access to model outputs (decisions and/or scores).
Based on different knowledge about SR models, we take into account three attack scenarios: 
white-box attack, query-based attack and transfer-based attack.
White-box attack relies on detailed information of the victim model, 
including internal architecture and learned parameters values.
Thus, a white-box attack adversary can easily and precisely computes 
the gradient of the loss w.r.t. the input by backpropagation.
On the contrary, black-box attack, including query-based and transfer-based attacks, 
assumes no knowledge about the model 
since the model is not transparently exposed to adversaries. 
Despite this, query-based attack can access the target model as an oracle, i.e., 
providing a series of carefully crafted inputs to the model and observing its outputs.
Transfer-based attack is based on adversarial transferability 
that adversarial examples crafted on one model remain effective for others. 
It is more practical in real-world applications yet more challenging 
since it cannot utilize the adaptive queries as in query-based attack.

% \begin{table}[t]
%     \begin{tabular}{}
        
%     \end{tabular}
% \end{table}

==> useless_results.tex <==
% absolute & change
\begin{table*}[htbp]
    \centering
    \caption{Transferability of the adversarial examples crafted by the BIM attack. 
    For each pair of source and target systems, we report the best result among all the \#iterations of BIM. 
    For each target system, the left column represents the absolute adversarial accuracy 
    while the right one indicates the relative accuracy drop under attack to that under No Attack.}
    \resizebox{\textwidth}{!}{%
      \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \midrule
      \multicolumn{1}{|c|}{\diagbox{\bf Source}{\bf Accuracy (\%)}{\bf Target}} & \multicolumn{2}{c|}{\textbf{iv\_plda}} & \multicolumn{2}{c|}{\textbf{xv\_plda}} & 
      \multicolumn{2}{c|}{\textbf{ecapa\_tdnn}} & \multicolumn{2}{c|}{\textbf{xv\_coss}} & \multicolumn{2}{c|}{\textbf{audionet}} & 
      \multicolumn{2}{c|}{\textbf{resnet18\_iden}} & \multicolumn{2}{c|}{\textbf{resnet18\_veri}} & \multicolumn{2}{c|}{\textbf{resnet34\_iden}} & 
      \multicolumn{2}{c|}{\textbf{resnet34\_veri}} & \multicolumn{2}{c|}{\textbf{autospeech\_iden}} & \multicolumn{2}{c|}{\textbf{autospeech\_veri}} & 
      \multicolumn{2}{c|}{\textbf{ge2e}} & \multicolumn{2}{c|}{\textbf{sincnet}} & \multicolumn{2}{c|}{\textbf{hubert\_large}} \\
      \midrule
      \textbf{No Attack} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{99.9} & \multicolumn{2}{c|}{96.4} & \multicolumn{2}{c|}{99.9} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{99.9} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{99.8} & \multicolumn{2}{c|}{58.8} & \multicolumn{2}{c|}{99.3} & \multicolumn{2}{c|}{78.7} & \multicolumn{2}{c|}{96.3} & \multicolumn{2}{c|}{95.2} \\
      \midrule
      \textbf{iv\_plda} & 0 & 100 & 69.5 & \textcolor{blue}{\bf 30.5} & 92.6 & 7.3 & 69.7 & \textcolor{blue}{\bf 26.7} & 87 & 12.9 & 99.5 & \textcolor{red}{\bf 0.5} & 99.3 & \textcolor{red}{\bf 0.6} & 96.8 & 3.2 & 96.9 & \textcolor{red}{\bf 2.9} & 47.8 & 11 & 92.5 & 6.8 & 63.1 & 15.6 & 93.3 & 3 & 62.3 & \textcolor{blue}{\bf 32.9} \\
      \midrule
      \textbf{xv\_plda} & 55.6 & \textcolor{blue}{\bf 44.4} & 0 & 100 & 77.4 & 22.5 & 62 & \textcolor{blue}{\bf 34.4} & 92 & 7.9 & 98.7 & \textcolor{red}{\bf 1.3} & 98.7 & \textcolor{red}{\bf 1.2} & 95.8 & 4.2 & 97.3 & 2.5 & 46 & 12.8 & 91.1 & 8.2 & 68.6 & 10.1 & 94.1 & \textcolor{red}{\bf 2.2} & 62.6 & \textcolor{blue}{\bf 32.6} \\
      \midrule
      \textbf{ecapa\_tdnn} & 91.4 & 8.6 & 85.7 & \textcolor{blue}{\bf 14.3} & 0 & 99.9 & 85 & 11.4 & 94.2 & 5.7 & 98.9 & \textcolor{red}{\bf 1.1} & 98.9 & \textcolor{red}{\bf 1} & 92.9 & 7.1 & 98.4 & \textcolor{red}{\bf 1.4} & 46.3 & \textcolor{blue}{\bf 12.5} & 89.8 & 9.5 & 71.4 & 7.3 & 94.7 & 1.6 & 66.4 & \textcolor{blue}{\bf 28.8} \\
      \midrule
      \textbf{xv\_coss} & 48.5 & \textcolor{blue}{\bf 51.5} & 41.4 & \textcolor{blue}{\bf 58.6} & 57.2 & \textcolor{blue}{\bf 42.7} & 0 & 96.4 & 89.9 & 10 & 98.1 & \textcolor{red}{\bf 1.9} & 97.8 & \textcolor{red}{\bf 2.1} & 93 & 7 & 92.3 & 7.5 & 43 & 15.8 & 85.1 & 14.2 & 62.2 & 16.5 & 93.4 & \textcolor{red}{\bf 2.9} & 69.7 & 25.5 \\
      \midrule
      \textbf{audionet} & 95.7 & 4.3 & 99.5 & \textcolor{red}{\bf 0.5} & 99.8 & \textcolor{red}{\bf 0.1} & 99.2 & \textcolor{red}{\bf -2.8} & 0 & 99.9 & 99.1 & 0.9 & 99.2 & 0.7 & 96 & 4 & 97 & 2.8 & 50.6 & \textcolor{blue}{\bf 8.2} & 95.3 & 4 & 66.4 & \textcolor{blue}{\bf 12.3} & 93.4 & 2.9 & 69 & \textcolor{blue}{\bf 26.2} \\
      \midrule
      \textbf{resnet18\_iden} & 98.6 & 1.4 & 99.6 & \textcolor{red}{\bf 0.4} & 99.8 & \textcolor{red}{\bf 0.1} & 99.3 & \textcolor{red}{\bf -2.9} & 93.4 & 6.5 & 0 & 100 & 65.7 & \textcolor{blue}{\bf 34.2} & 58.2 & \textcolor{blue}{\bf 41.8} & 58.4 & \textcolor{blue}{\bf 41.4} & 34.9 & 23.9 & 72 & 27.3 & 70.8 & 7.9 & 94.2 & 2.1 & 78.5 & 16.7 \\
      \midrule
      \textbf{resnet18\_veri} & 98 & 2 & 99.7 & \textcolor{red}{\bf 0.3} & 99.7 & \textcolor{red}{\bf 0.2} & 99.4 & \textcolor{red}{\bf -3} & 93.3 & 6.6 & 63.4 & \textcolor{blue}{\bf 36.6} & 0 & 99.9 & 52.8 & \textcolor{blue}{\bf 47.2} & 51.1 & \textcolor{blue}{\bf 48.7} & 30.3 & 28.5 & 64.5 & 34.8 & 69.7 & 9 & 94.2 & 2.1 & 76.2 & 19 \\
      \midrule
      \textbf{resnet34\_iden} & 98.8 & 1.2 & 99.7 & \textcolor{red}{\bf 0.3} & 99.8 & \textcolor{red}{\bf 0.1} & 99.6 & \textcolor{red}{\bf -3.2} & 95.5 & 4.4 & 84.8 & 15.2 & 79.9 & \textcolor{blue}{\bf 20} & 0 & 100 & 72.7 & \textcolor{blue}{\bf 27.1} & 40.6 & 18.2 & 76.7 & \textcolor{blue}{\bf 22.6} & 71.3 & 7.4 & 94.5 & 1.8 & 78.3 & 16.9 \\
      \midrule
      \textbf{resnet34\_veri} & 98.4 & 1.6 & 99.8 & \textcolor{red}{\bf 0.2} & 99.7 & \textcolor{red}{\bf 0.2} & 99.7 & \textcolor{red}{\bf -3.3} & 93.7 & 6.2 & 80 & 20 & 75 & \textcolor{blue}{\bf 24.9} & 61.1 & \textcolor{blue}{\bf 38.9} & 0 & 99.8 & 35.4 & 23.4 & 70.9 & \textcolor{blue}{\bf 28.4} & 70.2 & 8.5 & 94.1 & 2.2 & 78.6 & 16.6 \\
      \midrule
      \textbf{autospeech\_iden} & 97.4 & 2.6 & 99.6 & \textcolor{red}{\bf 0.4} & 99.8 & \textcolor{red}{\bf 0.1} & 99.5 & \textcolor{red}{\bf -3.1} & 95.9 & 4 & 90.6 & 9.4 & 89.7 & 10.2 & 82 & 18 & 76.3 & \textcolor{blue}{\bf 23.5} & 0 & 58.8 & 52 & \textcolor{blue}{\bf 47.3} & 72.3 & 6.4 & 94.4 & 1.9 & 77.2 & \textcolor{blue}{\bf 18} \\
      \midrule
      \textbf{autospeech\_veri} & 97.4 & 2.6 & 98.9 & \textcolor{red}{\bf 1.1} & 99.3 & \textcolor{red}{\bf 0.6} & 98.6 & \textcolor{red}{\bf -2.2} & 93.5 & 6.4 & 87.9 & 12.1 & 82.1 & 17.8 & 74.8 & \textcolor{blue}{\bf 25.2} & 68 & \textcolor{blue}{\bf 31.8} & 14.6 & \textcolor{blue}{\bf 44.2} & 0 & 99.3 & 70.1 & 8.6 & 94 & 2.3 & 76.4 & 18.8 \\
      \midrule
      \textbf{ge2e} & 96.5 & 3.5 & 99.7 & \textcolor{red}{\bf 0.3} & 99.8 & \textcolor{red}{\bf 0.1} & 99.1 & \textcolor{red}{\bf -2.7} & 74.7 & \textcolor{blue}{\bf 25.2} & 98.9 & 1.1 & 96.7 & 3.2 & 97.9 & 2.1 & 94.6 & 5.2 & 46.7 & \textcolor{blue}{\bf 12.1} & 89.7 & 9.6 & 10 & 68.7 & 92.6 & 3.7 & 69.3 & \textcolor{blue}{\bf 25.9} \\
      \midrule
      \textbf{sincnet} & 95.5 & 4.5 & 99.3 & \textcolor{red}{\bf 0.7} & 99.4 & \textcolor{red}{\bf 0.5} & 92.2 & 4.2 & 79.1 & \textcolor{blue}{\bf 20.8} & 97.8 & \textcolor{red}{\bf 2.2} & 96.3 & 3.6 & 93.7 & 6.3 & 93.9 & 5.9 & 44.8 & \textcolor{blue}{\bf 14} & 90.6 & 8.7 & 42.1 & \textcolor{blue}{\bf 36.6} & 28.7 & 67.6 & 85 & 10.2 \\
      \midrule
      \textbf{hubert\_large} & 98.3 & 1.7 & 99.9 & 0.1 & 99.6 & 0.3 & 99.6 & \textcolor{red}{\bf -3.2} & 96.7 & 3.2 & 99.9 & 0.1 & 100 & \textcolor{red}{\bf -0.1} & 99.4 & 0.6 & 99.8 & \textcolor{red}{\bf 0} & 50 & \textcolor{blue}{\bf 8.8} & 94 & \textcolor{blue}{\bf 5.3} & 74.4 & \textcolor{blue}{\bf 4.3} & 96 & 0.3 & 0 & 95.2 \\
      \bottomrule
      \end{tabular}%
    }
    \label{tab:transfer-BIM-best}%
  \end{table*}%

%%%% only-change-transpose
\begin{table*}[htbp]
    \centering
    \caption{Transferability of the adversarial examples crafted by the BIM attack. 
    For each pair of source and target systems, we report the best transferability result among all the \#iterations of BIM. 
    The results indicate the relative accuracy drop of the target systems compared to their benign accuracy.}
    \resizebox{\textwidth}{!}{%
      \begin{tabular}{|c|c||c|c|c||c|c|c|c|c|c|c|c||c||c|}
      \midrule 
      \diagbox{\bf Source}{\bf $\Downarrow$ Accuracy (\%)}{\bf Target} & \textbf{iv\_plda} & \textbf{ecapa\_tdnn} & \textbf{xv\_plda} & \textbf{xv\_coss} & \textbf{audionet} & \textbf{sincnet} & \textbf{resnet18\_iden} & \textbf{resnet18\_veri} & \textbf{resnet34\_iden} & \textbf{resnet34\_veri} & \textbf{autospeech\_iden} & \textbf{autospeech\_veri} & \textbf{ge2e} & \textbf{hubert\_large} \\
      \midrule
      \textbf{iv\_plda} & \cellcolor{gray!40} 100 & 8.6 & \textcolor{blue}{\bf 44.4} & \textcolor{blue}{\bf 51.5} & 4.3 & 4.5 & 1.4 & 2 & 1.2 & 1.6 & 2.6 & 2.6 & 3.5 & 1.7 \\
      \midrule
      \midrule
      \textbf{ecapa\_tdnn} & 7.3 & \cellcolor{gray!40} 99.9 & 22.5 & \textcolor{blue}{\bf 42.7} & \textcolor{red}{\bf 0.1} & \textcolor{red}{\bf 0.5} & \textcolor{red}{\bf 0.1} & \textcolor{red}{\bf 0.2} & \textcolor{red}{\bf 0.1} & \textcolor{red}{\bf 0.2} & \textcolor{red}{\bf 0.1} & \textcolor{red}{\bf 0.6} & \textcolor{red}{\bf 0.1} & 0.3 \\
      \midrule
      \textbf{xv\_plda} & \textcolor{blue}{\bf 30.5} & \textcolor{blue}{\bf 14.3} & \cellcolor{gray!40} 100 & \textcolor{blue}{\bf 58.6} & \textcolor{red}{\bf 0.5} & \textcolor{red}{\bf 0.7} & \textcolor{red}{\bf 0.4} & \textcolor{red}{\bf 0.3} & \textcolor{red}{\bf 0.3} & \textcolor{red}{\bf 0.2} & \textcolor{red}{\bf 0.4} & \textcolor{red}{\bf 1.1} & \textcolor{red}{\bf 0.3} & 0.1 \\
      \midrule
      \textbf{xv\_coss} & \textcolor{blue}{\bf 26.7} & 11.4 & \textcolor{blue}{\bf 34.4} & \cellcolor{gray!40} 96.4 & \textcolor{red}{\bf -2.8} & 4.2 & \textcolor{red}{\bf -2.9} & \textcolor{red}{\bf -3} & \textcolor{red}{\bf -3.2} & \textcolor{red}{\bf -3.3} & \textcolor{red}{\bf -3.1} & \textcolor{red}{\bf -2.2} & \textcolor{red}{\bf -2.7} & \textcolor{red}{\bf -3.2} \\
      \midrule
      \midrule
      \textbf{audionet} & 12.9 & 5.7 & 7.9 & 10 & \cellcolor{gray!40} 99.9 & \textcolor{blue}{\bf 20.8} & 6.5 & 6.6 & 4.4 & 6.2 & 4 & 6.4 & \textcolor{blue}{\bf 25.2} & 3.2 \\
      \midrule
      \textbf{sincnet} & 3 & 1.6 & \textcolor{red}{\bf 2.2} & \textcolor{red}{\bf 2.9} & 2.9 & \cellcolor{gray!40} 67.6 & 2.1 & 2.1 & 1.8 & 2.2 & 1.9 & 2.3 & 3.7 & 0.3 \\
      \midrule
      \textbf{resnet18\_iden} & \textcolor{red}{\bf 0.5} & \textcolor{red}{\bf 1.1} & \textcolor{red}{\bf 1.3} & \textcolor{red}{\bf 1.9} & 0.9 & \textcolor{red}{\bf 2.2} & \cellcolor{gray!40} 100 & \textcolor{blue}{\bf 36.6} & 15.2 & 20 & 9.4 & 12.1 & 1.1 & 0.1 \\
      \midrule
      \textbf{resnet18\_veri} & \textcolor{red}{\bf 0.6} & \textcolor{red}{\bf 1} & \textcolor{red}{\bf 1.2} & \textcolor{red}{\bf 2.1} & 0.7 & 3.6 & \textcolor{blue}{\bf 34.2} & \cellcolor{gray!40} 99.9 & \textcolor{blue}{\bf 20} & \textcolor{blue}{\bf 24.9} & 10.2 & 17.8 & 3.2 & \textcolor{red}{\bf -0.1} \\
      \midrule
      \textbf{resnet34\_iden} & 3.2 & 7.1 & 4.2 & 7 & 4 & 6.3 & \textcolor{blue}{\bf 41.8} & \textcolor{blue}{\bf 47.2} & \cellcolor{gray!40} 100 & \textcolor{blue}{\bf 38.9} & \textcolor{blue}{\bf 18} & \textcolor{blue}{\bf 25.2} & 2.1 & 0.6 \\
      \midrule
      \textbf{resnet34\_veri} & \textcolor{red}{\bf 2.9} & \textcolor{red}{\bf 1.4} & 2.5 & 7.5 & 2.8 & 5.9 & \textcolor{blue}{\bf 41.4} & \textcolor{blue}{\bf 48.7} & \textcolor{blue}{\bf 27.1} & \cellcolor{gray!40} 99.8 & \textcolor{blue}{\bf 23.5} & \textcolor{blue}{\bf 31.8} & 5.2 & \textcolor{red}{\bf 0} \\
      \midrule
      \textbf{autospeech\_iden} & 11 & \textcolor{blue}{\bf 12.5} & 12.8 & 15.8 & \textcolor{blue}{\bf 8.2} & \textcolor{blue}{\bf 14} & 23.9 & 28.5 & 18.2 & 23.4 & \cellcolor{gray!40} 58.8 & \textcolor{blue}{\bf 44.2} & \textcolor{blue}{\bf 12.1} & \textcolor{blue}{\bf 8.8} \\
      \midrule
      \textbf{autospeech\_veri} & 6.8 & 9.5 & 8.2 & 14.2 & 4 & 8.7 & 27.3 & 34.8 & \textcolor{blue}{\bf 22.6} & \textcolor{blue}{\bf 28.4} & \textcolor{blue}{\bf 47.3} & \cellcolor{gray!40} 99.3 & 9.6 & \textcolor{blue}{\bf 5.3} \\
      \midrule
      \midrule
      \textbf{ge2e} & 15.6 & 7.3 & 10.1 & 16.5 & \textcolor{blue}{\bf 12.3} & \textcolor{blue}{\bf 36.6} & 7.9 & 9 & 7.4 & 8.5 & 6.4 & 8.6 & \cellcolor{gray!40} 68.7 & \textcolor{blue}{\bf 4.3} \\
      \midrule
      \midrule
      \textbf{hubert\_large} & \textcolor{blue}{\bf 32.9} & \textcolor{blue}{\bf 28.8} & \textcolor{blue}{\bf 32.6} & 25.5 & \textcolor{blue}{\bf 26.2} & 10.2 & 16.7 & 19 & 16.9 & 16.6 & 18 & 18.8 & \textcolor{blue}{\bf \bf 25.9} & \cellcolor{gray!40} 95.2 \\
      \bottomrule
      \end{tabular}%
    }
    \label{tab:transfer-BIM-best}%
  \end{table*}%


% Table generated by Excel2LaTeX from sheet 'model_info'
\begin{table*}[t]
    \centering
    \caption{The detail of SR systems involved in transferability analysis.}
    \resizebox{\textwidth}{!}{%
      \begin{tabular}{|c|c|c|c|c|c|c|c|}
      \toprule
    % & \textbf{Input} & \multicolumn{1}{p{4.135em}|}{\textbf{Scoring Backend}} & \multicolumn{1}{p{7.545em}|}{\textbf{Training \newline{}Loss}} & \multicolumn{1}{p{8.09em}|}{\textbf{Learning \newline{}Method}} & \multicolumn{1}{p{7.545em}|}{\textbf{Model \newline{}Type}} & \textbf{Corpus} & \textbf{Structure} \\
      \diagbox{\bf System}{\bf Category} & \textbf{Input} & \textbf{Scoring Backend} & \textbf{Training Loss} & \textbf{Learning Method} & \textbf{Model Type} & \textbf{Corpus} & \textbf{Structure} \\
      \midrule
      \textbf{iv\_plda}~\cite{kaldi-ivector-plda} & mfcc & PLDA & & unsupervised & Generative & VoxCeleb1+VoxCeleb2 & GMM \\
      \midrule
      \midrule
      \textbf{ecapa\_tdnn}~\cite{ECAPA-TDNN} & fbank & COSS & classification & supervised & Discriminitive & VoxCeleb1 & TDNN \\
      \midrule
      \textbf{xv\_plda}~\cite{kaldi-xvector-plda} & mfcc & PLDA & classification & supervised & Discriminitive & VoxCeleb1+VoxCeleb2 & TDNN \\
      \midrule
      \textbf{xv\_coss}~\cite{xv_coss,speech-brain} & fbank & COSS & classification & supervised & Discriminitive & VoxCeleb1 & TDNN \\
      \midrule
      \midrule
    %   \textbf{audionet}~\cite{becker2018interpreting} & mfcc & COSS & classification & supervised & Discriminitive & LibriSpeech & 1-D CNN \\
    %   \midrule
    %   \textbf{resnet18\_iden}~\cite{resnet18} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & 2D-CNN \\
    %   \midrule
    %   \textbf{resnet18\_veri}~\cite{resnet18} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & 2D-CNN \\
    %   \midrule
    %   \textbf{resnet34\_iden}~\cite{resnet34} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & 2D-CNN \\
    %   \midrule
    %   \textbf{resnet34\_veri}~\cite{resnet34} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & 2D-CNN \\
    %   \midrule
    %   \textbf{autospeech\_iden}~\cite{auto-speech} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & 2D-CNN \\
    %   \midrule
    %   \textbf{autospeech\_veri}~\cite{auto-speech} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & 2D-CNN \\
      \textbf{audionet}~\cite{becker2018interpreting} & fbank & COSS & classification & supervised & Discriminitive & LibriSpeech & CNN \\
      \midrule
      %   \textbf{sincnet}~\cite{SincNet} & wavform & COSS & classification & supervised & Discriminitive & TIMIT & 1D-CNN \\
      \textbf{sincnet}~\cite{SincNet} & wavform & COSS & classification & supervised & Discriminitive & TIMIT & CNN \\
      \midrule
      \textbf{resnet18\_iden}~\cite{resnet18} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & CNN \\
      \midrule
      \textbf{resnet18\_veri}~\cite{resnet18} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & CNN \\
      \midrule
      \textbf{resnet34\_iden}~\cite{resnet34} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & CNN \\
      \midrule
      \textbf{resnet34\_veri}~\cite{resnet34} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & CNN \\
      \midrule
      \textbf{autospeech\_iden}~\cite{auto-speech} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & CNN \\
      \midrule
      \textbf{autospeech\_veri}~\cite{auto-speech} & spectrogram & COSS & classification & supervised & Discriminitive & VoxCeleb1 & CNN \\
      \midrule
      \midrule
      \textbf{ge2e}~\cite{GE2E} & fbank & COSS & verification & supervised & Discriminitive & TIMIT & LSTM \\
      \midrule
      \midrule
      \textbf{hubert\_large}~\cite{HuBert,SUPERB} & wavform & COSS & & self-supervised & & LibriLight & CNN+Transformer \\
      \bottomrule
      \end{tabular}%
    }
    \label{tab:system-info}%
  \end{table*}%

  % \begin{table*}[htbp]
%     \centering
%     \caption{Results of over-the-air attack.}
%     \resizebox{\textwidth}{!}{%
%       \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%       \toprule
%       \multirow{3}[6]{*}{} & \multirow{3}[6]{*}{$\mathbf{\varepsilon}$} & \multirow{3}[6]{*}{\textbf{MOS-LQO}} & \multicolumn{2}{c|}{\textbf{Reverberation}} & \multicolumn{20}{c|}{\textbf{Ambient Noise}} \\
%   \cmidrule{4-25}          &       &       & \multirow{2}[4]{*}{\textbf{Sim.}} & \textbf{Real} & \multicolumn{5}{c|}{\textbf{White Noise}} & \multicolumn{5}{c|}{\textbf{Point Source Noise}} & \multicolumn{5}{c|}{\textbf{Music Noise}} & \multicolumn{5}{c|}{\textbf{Speech Babble Noise}} \\
%   \cmidrule{5-25}          &       &       &       & \textbf{+Equ. Dist.} & \textbf{20} & \textbf{15} & \textbf{10} & \textbf{5} & \textbf{0} & \textbf{20} & \textbf{15} & \textbf{10} & \textbf{5} & \textbf{0} & \textbf{20} & \textbf{15} & \textbf{10} & \textbf{5} & \textbf{0} & \textbf{20} & \textbf{15} & \textbf{10} & \textbf{5} & \textbf{0} \\
%       \midrule
%       \multirow{3}[6]{*}{} & 0.03  & 1.63  & 2.6   & 4.9   & 0.8   & 8.9   & 36.5  & 72.7  & 93.2  & 0.2   & 1.6   & 5.9   & 12.3  & 22.6  & 0     & 0.2   & 1.8   & 4.8   & 11.1  & 0     & 0     & 0.2   & 3.2   & 7.2 \\
%   \cmidrule{2-25}          & 0.04  & 1.48  & 0.9   & 3.9   & 0.1   & 5.7   & 18    & 58.8  & 85.8  & 0     & 0.6   & 2.6   & 8.3   & 17    & 0     & 0     & 0.5   & 2.3   & 7.8   & 0     & 0     & 0.1   & 0.8   & 3.1 \\
%   \cmidrule{2-25}          & 0.05  & 1.38  & 0.7   & 2.8   & 0     & 2.5   & 10.9  & 44.7  & 76.7  & 0     & 0.2   & 2.2   & 6.9   & 13.7  & 0     & 0     & 0.2   & 1.8   & 5.7   & 0     & 0     & 0.1   & 0.9   & 3.5 \\
%       \midrule
%       \multirow{3}[6]{*}{\textbf{Sim. RIR}} & 0.01  & 1.88  & 0     & 0     & 0     & 1.5   & 15.1  & 53    & 76.7  & 0.1   & 0.3   & 1.4   & 4.2   & 12.1  & 0     & 0     & 0.1   & 1.3   & 3     & 0     & 0     & 0     & 0.1   & 0.7 \\
%   \cmidrule{2-25}          & 0.02  & 1.56  & 0     & 0     & 0     & 0     & 0.7   & 16.7  & 57.1  & 0     & 0     & 0.2   & 1.4   & 5.2   & 0     & 0     & 0     & 0.1   & 0.5   & 0     & 0     & 0     & 0     & 0.2 \\
%   \cmidrule{2-25}          & 0.03  & 1.40  & 0     & 0     & 0     & 0     & 0     & 3.7   & 35.2  & 0     & 0     & 0     & 1     & 2.7   & 0     & 0     & 0     & 0     & 0.1   & 0     & 0     & 0     & 0     & 0 \\
%   \midrule
%   {\bf White Noise} & 0.01 & 1.55 & 0 & 0.1& 0& 0& 0& 1.3& 7.4& 0& 0& 0& 0.2& 1.1& 0& 0& 0& 0& 0.4& 0& 0& 0& 0& 0.1 \\  
%   \bottomrule
%    \end{tabular}%
%     }
%     \label{tab:over-the-air}%
%   \end{table*}%
% Table generated by Excel2LaTeX from sheet 'Sheet1'

% \begin{table*}[htbp]
%     \centering
%     \caption{Add caption}
%     \resizebox{1.0\textwidth}{!}{%
%       \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%       \toprule
%       \multirow{4}[8]{*}{} & \multicolumn{10}{c|}{\textbf{CSI}}                                            & \multicolumn{3}{c|}{\textbf{SV}} \\
%   \cmidrule{2-14}          & \multicolumn{2}{c|}{\textbf{Untargeted}} & \multicolumn{4}{c|}{\textbf{Targeted Random}} & \multicolumn{4}{c|}{\textbf{Targeted Least Likely}} & \multicolumn{3}{c|}{\textbf{Targeted}} \\
%   \cmidrule{2-14}          & \multicolumn{2}{c|}{\textbf{Asr (\%)}} & \multicolumn{2}{c|}{\textbf{Asr (\%)}} & \multicolumn{2}{c|}{\textbf{Mis (\%)}} & \multicolumn{2}{c|}{\textbf{Asr (\%)}} & \multicolumn{2}{c|}{\textbf{Mis (\%)}} & \multicolumn{3}{c|}{\textbf{Asr (\%)}} \\
%   \cmidrule{2-14}          & $f_\text{CE}$ & $f_\text{M}^{1}$ & \multicolumn{1}{l|}{$f_\text{CE}$} & \multicolumn{1}{l|}{$f_\text{M}^{2}$} & \multicolumn{1}{l|}{$f_\text{CE}$} & \multicolumn{1}{l|}{$f_\text{M}^{2}$} & \multicolumn{1}{l|}{$f_\text{CE}$} & \multicolumn{1}{l|}{$f_\text{M}^{2}$} & \multicolumn{1}{l|}{$f_\text{CE}$} & \multicolumn{1}{l|}{$f_\text{M}^{2}$} & $f_\text{BCE}$ & \multicolumn{1}{l|}{$f_\text{M}^{3}$} & \multicolumn{1}{l|}{$f_\text{M}^{4}$} \\
%       \midrule
%       \boldmath{}\textbf{$s\in D\setminus\{-1\}$}\unboldmath{} & 28.2  & 28.2  & 13.6  & \textcolor{blue}{\textbf{23.3}} & 13.6  & \textcolor{blue}{\textbf{25.7}} & 1.3   & \textcolor{blue}{\textbf{4.9}} & 1.6   & \textcolor{blue}{\textbf{9.9}} & 68.7  & 68.7  & \xmark \\
%       \midrule
%       \boldmath{}\textbf{$s = -1$}\unboldmath{} & \multicolumn{2}{c|}{---} & \textcolor{blue}{\textbf{81.6}} & 70.7  & 100   & 100   & \textcolor{blue}{\textbf{57}} & 36.6  & 100   & 100   & 56.9  & \xmark & 56.9 \\
%       \bottomrule
%       \end{tabular}%
%     }
%     \label{tab:addlabel}%
%   \end{table*}%

%   \begin{table*}[htbp]
%     \centering
%     \caption{Add caption}
%     \resizebox{1.0\textwidth}{!}{%
%       \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%       \toprule
%       \multirow{3}[6]{*}{} & \multicolumn{5}{c|}{\textbf{Untargeted}} & 
%       \multicolumn{8}{c|}{\begin{tabular}[c]{@{}c@{}}\boldmath{}\textbf{Targeted Random}\unboldmath{} \\ {\boldmath{}\bf ($t\neq -1$) \unboldmath{}}\end{tabular}} & 
%       \multicolumn{8}{c|}{\begin{tabular}[c]{@{}c@{}}\boldmath{}\textbf{Targeted Least Likely}\unboldmath{} \\ {\boldmath{}\bf ($t\neq -1$) \unboldmath{}} \end{tabular}} & 
%       \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}\boldmath{}\textbf{Targeted}\unboldmath{} \\ {\boldmath{}\bf ($t=-1$) \unboldmath{}} \end{tabular}} \\
%   \cmidrule{2-24}          & \multicolumn{5}{c|}{\textbf{Asr (\%)}}     & \multicolumn{4}{c|}{\textbf{Asr (\%)}} & \multicolumn{4}{c|}{\textbf{Mis (\%)}} & \multicolumn{4}{c|}{\textbf{Asr (\%)}} & \multicolumn{4}{c|}{\textbf{Mis (\%)}} & \multicolumn{2}{c|}{\textbf{Asr (\%)}} \\
%   \cmidrule{2-24}          & $f_\text{CE}$ & $f_{\tt min}^{5,6}$ & $f_{\tt min}^{5,1}$ & $f_{\tt min}^{5,10}$ & $f_\text{M}^{8}$ & $f_\text{CE}$ & $f_\text{M}^{7}$ & $f_\text{M}^{2}$ & $f_\text{M}^{9}$ & $f_\text{CE}$ & $f_\text{M}^{7}$ & $f_\text{M}^{2}$ & $f_\text{M}^{9}$ & $f_\text{CE}$ & $f_\text{M}^{7}$ & $f_\text{M}^{2}$ & $f_\text{M}^{9}$ & $f_\text{CE}$ & $f_\text{M}^{7}$ & $f_\text{M}^{2}$ & $f_\text{M}^{9}$ & \multicolumn{2}{c|}{$f_\text{M}^{5}$} \\
%       \midrule
%       \boldmath{}\textbf{$s\in D\setminus\{-1\}$}\unboldmath{} & 80.1  & \textcolor{blue}{\textbf{83.9}} & \textcolor{blue}{\textbf{83.9}} & 69.5  & \xmark & \textcolor{blue}{\textbf{9.7}} & 9.4   & 9.2   & 9.4   & 30.6  & \textcolor{blue}{\textbf{62.8}} & \textcolor{blue}{\textbf{62.8}} & 22.3  & 0.1   & 0     & 0     & \textcolor{blue}{\textbf{0.3}} & 27.4  & \textcolor{blue}{\textbf{61.8}} & \textcolor{blue}{\textbf{61.8}} & 14.8  & 83.9  & 83.9 \\
%       \midrule
%       \boldmath{}\textbf{$s = -1$}\unboldmath{} & \xmark & \xmark & \xmark & \xmark & 95    & 26    & 33.9  & 10.8  & \textcolor{blue}{\textbf{34.3}} & 26.1  & 34.9  & 10.8  & \textcolor{blue}{\textbf{35.4}} & 0.4   & 2.1   & 0.1   & \textcolor{blue}{\textbf{2.2}} & 0.4   & 2.4   & 0.1   & \textcolor{blue}{\textbf{2.9}} & \multicolumn{2}{c|}{---} \\
%       \bottomrule
%       \end{tabular}%
%     }
%     \label{tab:addlabel}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'S-T-CSI'

% Table generated by Excel2LaTeX from sheet 'basic attack'
% \begin{table}[htbp]
%     \centering
%     \caption{Results of White-box and query-based black-box attacks.}
%     \resizebox{0.5\textwidth}{!}{%
%       \begin{tabular}{|c|c|c|c|c|c|}
%       \toprule
%       \multicolumn{2}{|c|}{\multirow{2}[4]{*}{\bf Attack}} & \multicolumn{1}{c|}{\bf Effectiveness} & \multicolumn{3}{c|}{\bf Stealthiness} \\
%   \cmidrule{3-6}    \multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\bf Asr} & \multicolumn{1}{c|}{\bf L2} & \multicolumn{1}{c|}{\bf SNR} & \multicolumn{1}{c|}{\bf MOS-LQO} \\
%       \midrule
%       \multicolumn{2}{|c|}{\bf FGSM} & \multicolumn{1}{c|}{28.2} & \multicolumn{1}{c|}{0.533} & \multicolumn{1}{c|}{28.61} & \multicolumn{1}{c|}{2.28} \\
%       \midrule
%       \multirow{3}[6]{*}{\bf BIM} & {\bf 2}     & \multicolumn{1}{c|}{90.8} & \multicolumn{1}{c|}{0.159} & \multicolumn{1}{c|}{39.13} & \multicolumn{1}{c|}{3.52} \\
%   \cmidrule{2-6}    \multicolumn{1}{|c|}{} & {\bf 3}     & \multicolumn{1}{c|}{99.9} & \multicolumn{1}{c|}{0.203} & \multicolumn{1}{c|}{37} & \multicolumn{1}{c|}{3.32} \\
%   \cmidrule{2-6}    \multicolumn{1}{|c|}{} & {\bf 4}     & \multicolumn{1}{c|}{100} & \multicolumn{1}{c|}{0.241} & \multicolumn{1}{c|}{35.5} & \multicolumn{1}{c|}{3.16} \\
%       \midrule
%       \multicolumn{2}{|c|}{\bf CW$_2$-0} & \multicolumn{1}{c|}{100} & \multicolumn{1}{c|}{0.057} & \multicolumn{1}{c|}{50.47} & \multicolumn{1}{c|}{4.17} \\
%       \midrule
%       \multicolumn{2}{|c|}{\bf FAKEBOB} & \multicolumn{1}{c|}{100} & \multicolumn{1}{c|}{0.436} & \multicolumn{1}{c|}{29.92} & \multicolumn{1}{c|}{2.55} \\
%       \midrule
%       \multicolumn{2}{|c|}{\bf SirenAttack} &       &       &       &  \\
%       \bottomrule
%       \end{tabular}%
%     }
%     \label{tab:basic-attack}%
%   \end{table}%
